Are Images Indistinguishable to Humans Also Indistinguishable to Classifiers?

The ultimate goal of generative models is to perfectly capture the data distribution. For image generation, common metrics of visual quality (e.g., FID) and the perceived truthfulness of generated images seem to suggest that we are nearing this goal. However, through distribution classification tasks, we reveal that, from the perspective of neural network-based classifiers, even advanced diffusion models are still far from this goal. Specifically, classifiers are able to consistently and effortlessly distinguish real images from generated ones across various settings. Moreover, we uncover an intriguing discrepancy: classifiers can easily differentiate between diffusion models with comparable performance (e.g., U-ViT-H vs. DiT-XL), but struggle to distinguish between models within the same family but of different scales (e.g., EDM2-XS vs. EDM2-XXL). Our methodology carries several important implications. First, it naturally serves as a diagnostic tool for diffusion models by analyzing specific features of generated data. Second, it sheds light on the model autophagy disorder and offers insights into the use of generated data: augmenting real data with generated data is more effective than replacing it. Third, classifier guidance can significantly enhance the realism of generated images.

==> sec/2_background.tex <==
\section{Background}
\subsection{Diffusion model}
Diffusion models~\citep{sohl2015deep, song2020score, ho2020denoising} gradually inject noise into data $\boldsymbol{x}$ during the forward process:
\begin{align}
    \boldsymbol{z}_t = \sqrt{\bar{\alpha}_t} \boldsymbol{x} + \sqrt{1 - \bar{\alpha}_t} \boldsymbol{\epsilon},
\end{align}
and remove noise to generate data in the reverse process. Diffusion models typically use a noise prediction network $\boldsymbol{\epsilon}_{\boldsymbol{\theta}}(\boldsymbol{z}_t, t)$ to predict the noise $\boldsymbol{\epsilon}$ added to $\boldsymbol{z}_t$. Noise prediction loss is defined as:
\begin{align}
\label{eq:loss_diffusion}
\mathcal{L} = \mathbb{E}_{t, \boldsymbol{x}_0, \boldsymbol{\epsilon}} [\|\boldsymbol{\epsilon}_{\boldsymbol{\theta}}(\boldsymbol{z}_t, t) - \boldsymbol{\epsilon}\|_2^2].
\end{align}

\subsection{Frequency filter}
\label{sec:frequency_filter}
The frequency content of an image represents the rate of pixel value changes. Low-frequency components capture overall shapes and gradual grayscale changes, while high-frequency components reflect fine details like edges and textures. Notably, convolutional neural networks can detect high-frequencies that are often imperceptible to humans~\citep{wang2020high}. In our paper, we implement a rectangular filter and discuss the choice of this filter in Appendix~\ref{app:choice_filter}.

\textbf{Low-pass filters} are implemented as follows: Compute the Fourier transform of the image \( f(x, y) \) using \( F(u, v) = \text{FFT}(f(x, y)) \), and then center the spectrum with \( F_c(u, v) = \text{fftshift}(F(u, v)) \). Define a rectangular mask \( H(u, v) \) in frequency domain, where $M$ and $N$ are the image dimensions:
\begin{align}
H(u, v) = 
\begin{cases} 
1 & \text{if } \left| u - \frac{M}{2} \right| \leq \text{threshold} \\ 
  & \quad \text{and } \left| v - \frac{N}{2} \right| \leq \text{threshold}, \\
0 & \text{otherwise}.
\end{cases}   
\end{align}
Apply the mask by multiplying \( G(u, v) = F_c(u, v) \odot H(u, v) \), reverse the shift with \( G_c(u, v) = \text{ifftshift}(G(u, v)) \), and transform back to the spatial domain using \( g(x, y) = \text{IFFT}(G_c(u, v)) \).

\textbf{High-pass filters} are implemented similarly, but with the mask defined to pass high frequencies:
\begin{align}
H(u, v) = 
\begin{cases} 
0 & \text{if } \left| u - \frac{M}{2} \right| \leq \text{threshold} \\ 
  & \quad \text{and } \left| v - \frac{N}{2} \right| \leq \text{threshold}, \\
1 & \text{otherwise}.
\end{cases}   
\end{align}

\textbf{Band-pass filters} combine low-pass and high-pass filters, allowing frequencies between low and high thresholds to pass while setting others to 0.

